On the Hardware Feasibility of Nonlinear Trajectory Optimization for Legged Locomotion based on a Simplified Dynamics

Simplified models are useful to increase the computational efficiency of a motion planning algorithm, but their lack of accuracy have to be managed. We propose two feasibility constraints to be included in a Single Rigid Body Dynamicsbased trajectory optimizer in order to obtain robust motions in challenging terrain. The first one finds an approximate relationship between joint-torque limits and admissible contact forces, without requiring the joint positions. The second one proposes a leg model to prevent leg collision with the environment. Such constraints have been included in a simplified nonlinear nonconvex trajectory optimization problem. We demonstrate the feasibility of the resulting motion plans both in simulation and on the Hydraulically actuated Quadruped (HyQ) robot, considering experiments on an irregular terrain.

==> sections/section2.tex <==
\subsection{Related Works}\label{sec:relatedWorks}

The trade-off between simplicity of the model and feasibility of a whole-body motion on rough terrain is still at the core of the research in robotic legged locomotion.
One approach consists in using the trajectory generated with \gls{cd} (which is typically lower dimensional than the full dynamic model of the robot) in combination with the full robot kinematics to obtain a feasible whole-body motion \cite{Dai2016d, Herzog2016}. A similar approach was used by Valenzuela \etal \cite{Valenzuela2016} in which the authors compute the sequence of footholds using a Mixed Integer Convex optimization problem and then solve a nonlinear problem to find a linear and angular centroidal momentum trajectory. Budhiraja \etal \cite{Budhiraja2019} generated a trajectory for the \gls{com}, in both the simplified and in the full dynamic model, making sure that the former is coherent with the latter. All these approaches have been only tested in simulation with a bipedal robot, but never on the robotic hardware.

Farshidian \etal \cite{Farshidian2017} have introduced a nonlinear \gls{mpc} which is able to compute the relevant motion quantities in a short amount of time suitable for interactive rates. The limit of this approach is that it requires a big computational effort and it can thus only plan few phases of the motion (\eg one step prediction horizon).

Other authors leave on the motion controller the burden to verify the whole-body feasibility of the motion plan and focus, instead, on the nonlinearities which are present in the \gls{cd} and \gls{srbd} formulations (mainly angular momentum and contact phases duration). These are usually tackled by either defining a convex relaxation of the formulation \cite{Dai2016b, Ponton2018}, or by predefining the feet position for the entire trajectory \cite{DiCarlo2018a}. 

%Convex problems are widely used, because they guarantee faster computations. \cite{Ding2018} convexifies the non-linear torque constraint such that it can be added to the model, \cite{DiCarlo2018a} uses a convex model predicitve control to determine ground reaction forces.

Winkler \etal \cite{Winkler2018} implemented a trajectory optimization, based on the \gls{srbd}, in which \gls{com} position, orientation, feet position, contact forces and their derivatives are concurrently optimized. The efficiency of this planner has been demonstrated both in simulation and on the real hardware on flat terrains. On rough terrains, however, only knowing the trajectory of the \gls{com} and the feet is not enough to obtain a feasible whole-body motion that can be deployed on the real robotic hardware as other feasibility constraints such as joint-torque limits and geometry of the robot's legs need to be considered.
%Since there are more than one configuration of the base that results in the same \gls{com} position, a unique solution for the joint configuration cannot be obtained in closed form. The base and joints trajectories then have to be computed by a suitable motion controller in accordance to the \gls{com} references provided by the planner.

A state-of-art approach to the problem of avoiding collision between legs and ground is looking for a collision-free swing phase, considering the height map of the terrain and the robot configuration \cite{Doshi2007}. An alternative is presented in \cite{Barasuol2019}, in which the controller is able to detect the point of application of the ground reaction forces from the foot to the shin in case of collision. This method can guarantee safe navigation on challenging terrains, however, it is a pure reactive module which does not increase the robustness of the planner.

The joint-torque limits constraint problem is usually only addressed at controller level \cite{Samy2017, Fahmi2019RAL}. In order to explicitly consider this limit at the planning stage, Ding \etal \cite{Ding2018} convexify the nonlinear joint-torque constraint such that it can be added to a Mixed Integer Quadratically Constrained Program (MIQCP). This formulation is suitable for convex optimization and it thus computationally efficient. The decision to employ a unique outer bounding ellipsoid as an approximation of the force ellipsoids, however, discards the important (configuration dependent) information regarding the relationship between the leg's configuration and shape of the force ellipsoids (\ie the contact force is constant and it does not depend on the foot position).

Orsolino \etal, instead, used the force polytopes \cite{Chiacchio1997} to map the joint-torques limits into a set of admissible centroidal wrenches \cite{Orsolino2018a} or \gls{com} positions \cite{Orsolino2018b}. The former approach however, is not suitable for online foothold optimization because of its computational effort while the latter is only suitable for static gaits.

